Peer Surveillance in Online Communities

Online communities are not safe spaces for user privacy. Even though existing research focuses on creating and improving various content moderation strategies and privacy preserving technologies, platforms hosting online communities support features allowing users to surveil one another--leading to harassment, personal data breaches, and offline harm. To tackle this problem, we introduce a new, work-in-progress framework for analyzing data privacy within vulnerable, identity-based online communities. Where current SOUPS papers study surveillance and longitudinal user data as two distinct challenges to user privacy, more work needs to be done in exploring the sites where surveillance and historical user data assemble. By synthesizing over 40 years of developments in the analysis of surveillance, we derive properties of online communities that enable the abuse of user data by fellow community members and suggest key steps to improving security for vulnerable users. Deploying this new framework on new and existing platforms will ensure that online communities are privacy-conscious and designed more inclusively.

==> reddit.tex <==
\section{Researching Reddit Communities}
\label{sec:reddit}

\Reddit communities provide researchers with an abundance of data on user reactions, relationships, and other social behavior.
Some analysis of \reddit examine how online behavior translates offline, such as Lu et. al who investigated changes in drug addiction by tracing users' paths into different subreddits~\cite{lu:sigkdd2019}.
However, certain behavior and conduct is specific within \reddit, and we will focus particularly on the emergent practices in individual communities and groups of communities.
In January 2023, we conducted a search on the ACM Full-Text Collection database \footnote{The ACM Digital Library collects all publications from the Association for Computing Machinery. We selected it to conduct our search because of the prevalence of \reddit in Human-Computer Interaction and Computer Supported Cooperative Work research}.
Excluded from this search were works from \textit{New Media \& Society} as well as \textit{Social Media and Society}.
Even though key works, such as Fatallah~\cite{fathallah:nms2022} and Gibson~\cite{gibson:sms2019}, are published at these venues, a majority of the work about \reddit is available on the ACM Digital Library.\footnote{Our search consisted of the following key terms: [All: reddit] AND [All: ``communit*" or ``group"] AND [All: ``behav*" or ``habit”].}
From 420 results, we identified 81 papers relating to user behavior in communities on \reddit and analyze them here.
By highlighting most commonly analyzed communities, we reveal that identity based communities remain understudied.
Then, by surveying different dynamics on the platform, we reveal that \reddit research examines only user to user relationships, individual user relationships, and external user to community relationships rather than relationships \textit{within} community contexts.

\subsection{Popular Communities}

By focusing on the most popular communities, analysis' of \reddit posit insights into the online experience of large groups with common interests.
A list of researched communities is provided in \autoref{tab:redditcommunities}.
Mall et al. characterize toxicity by analyzing users across \reddit regardless of the communities and context in which users' comments were made~\cite{mall:hci2020}.
This popular approach~\cite{kotenko:idaacs2021,koncar:aws2021,decandia:aws2022,thukral:asnam2020}, of taking large samples across \reddit, misunderstands that each \reddit community is interchangeable when they are not.
Behaviors within political groups differ drastically from behavior on r/lgbt; the subreddits r/The\_Donald and r/hillaryclinton do not share the same vocabulary with general news communities whereas LGBTQ+ subreddits share similar language of minority stress ~\cite{jungherr:sscr2022,saha:cscw2019}.

\input{tables/redditcommunities.tex}

\subsubsection{Methods of Clustering Communities}

A large portion of \reddit research cluster communities that share similar interests, such as parenting \cite{sepahpour:www2022}, post-college~\cite{gong:cscw2021}, and work from home groups~\cite{cho:group2022}.
Even communities that share similar interests may diverge in small ways unnoticeable to an outsiders.
Members of the communities r/proED and r/loseit may both talk about weight loss, but their discussions carry different intentions~\cite{chancellor:hci2018}.
These nuances must be accounted for when studying similar communities to avoid misrepresenting users' experiences.
\Reddit's nature is inherently disparate; it is a platform constituted by contrasting, and often clashing, communities.
Deeper understanding gets lost when analyzing aggregated communities on \reddit because it is not a platform designed for universal experiences.
Moreover, Chandrasekharan et al. cluster communities based on similar comments removed~\cite{chandrasekharan:hci2018}.
Clustering communities this way ignores two other types of content: the content that remains after moderation and the other behavior-shaping tools available on \reddit.
Content that remains unmoderated on \reddit does impact the creation and evolution of community norms~\cite{chancellor:cscw2016, gerrard:nms2018}.
Additionally, tagging, upvoting, downvoting, positive replies, and negative replies all factor into what user’s post and what they think they should be posting on \Reddit~\cite{newell:aaai2021}.
In addition to highlighting removed content, analysing the content that remains after moderation and capturing the use of other platform features is necessary to understanding norm development in \Reddit communities.

\subsection{Identity-Based Communities}

Of the four identity based communities studied, Asian-American groups made up three results~\cite{dosono:hci2019,dosono:cscw2020,dosono:hci2018} while LGBTQ+ groups only appeared once~\cite{saha:cscw2019}.
Other sexual and gender identities are present in online self-disclosure research, yet these studies investigate how community features on platforms such as YouTube and Facebook interact with individual timelines and not how these communities interact on their own~\cite{green:bit2015,duguay:nms2016,haimson:fm2016,haimson:hci2016,ammari:cscw2016}.
Minorities within different national contexts also remain unexplored.
Structural issues in academic research, such as a focus on the issue of the day, illustrate why identity based communities are overlooked.
A large portion of \reddit research explores right-wing radicalization, misogyny, and conspiracy theories within communities---issues pushed to the forefront by the 2016 United States presidential election~\cite{habib:cscw2022,horta:cscw2021,mamie:aws2021, farrell:aws2019,farrell:aws2020,samory:cscw2018,massachs:aws2020,jungherr:sscr2022}.
Solving the problem of the day is important, but identity based communities often get knocked to the bottom of research agendas when politics and funding shuffles priorities.
The desire for large data sets also contributes to a lack of analysis on identity based communities.
\reddit research relies on tens and hundreds of thousands of comments, posts, and interactions~\cite{chandrasekharan:hci2018}.
It is impossible to create these large data sets with small, often inactive communities. 
As a result, more identity based communities remain to be studied on \reddit.

\subsection{Platform Dynamics}

Other dynamics and relationships remain understudied on \reddit beyond aggregate user to user interactions.
Eight distinct relationships emerged from previous \reddit research: moderators and platforms, users and platforms, users and moderators, moderator to moderator, user to user, individual user, user and community, community to community, and platform to community.
A definition of these terms is provided in \autoref{tab:redditdynamics}.

\subsubsection{User Relationships}

The two most studied dynamics were the user to user relationship and the individual user experience.
These studies focus on aggregating user to user interactions to demonstrate antisocial activity online, such as hate speech, toxicity, and the sharing of pornographic material~\cite{zannettou:aws2020, xia:cscw2020, park:cscw2022}.
Given the abundance of user to user research, few studies explore how communities affect user behavior \textit{within} those specific communities.
These studies typically center around health issues, such as mental health, weight, and addiction, and demonstrate how online communities change user's offline behavior~\cite{gauthier:hci2022,desanto:tsc2022,chancellor:hci2019,fettach:iiwbas2020,chancellor:hci2018, biester:atmis2021,sharma:hci2018}.
User behavior changes in these communities are seen physically, whereas changes in user individuality, temperament, and offline behavior remain elusive.

\input{tables/redditdynamics.tex}

\subsubsection{Moderator Relationships}

Moderators on \reddit are either the creators of the individual communities or volunteers chosen by existing moderators.\footnote{Unlike Facebook, where content moderators are paid employees of Facebook or a contractor, \Reddit moderators are members of the communities they moderate and work for free.}
In our search, the moderator to moderator relationship appeared the least.
Moderator hesitation and distrust might explain this gap to researchers interested in how moderators interact with one another.
Dosono and Semaan solicited requests to 118 moderators of Asian American and Pacific Islander communities, yet only twenty-one moderators became participants~\cite{dosono:hci2019}.

\subsubsection{Platform Relationships}

The moderator and platform relationship, the platform to community relationship, and the user to platform relationship are also underrepresented.
A lack of transparency cannot be blamed for ignoring how users, moderators and communities interact with \reddit at large.
\Reddit publishes a transparency report annually that quantifies their enforcement of the publicly available content policy and moderator code of conduct~\cite{tr:reddit,cp:reddit,mcoc:reddit}.
\reddit as a platform has experienced controversies and how users, moderators, and communities react all contribute to the evolution of group behavior on the platform~\cite{newell:aaai2021}.

==> tables/redditcommunities.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{| l | l |} 
\hline
\textbf{Subreddit} &  \textbf{Related Work}\\
\hline
Addiction Recovery Groups &~\cite{chancellor:hci2019,gauthier:hci2022}\\
\hline
r/AlphabayMarket &~\cite{hazel:sms2020}\\
\hline
r/AmItheAsshole &~\cite{decandia:aws2022}\\
\hline
r/AppalachinTrail &~\cite{kotut:hci2020}\\
\hline
Artificial Intelligence Groups &~\cite{ng:chb2022}\\
\hline
Asian Americans and Pacific Islanders &~\cite{dosono:hci2019,dosono:cscw2020,dosono:hci2018}\\
\hline
r/AskHistorians &~\cite{gruzd:cscw2020,gilbert:hci2020}\\
\hline
r/assholedesign &~\cite{gray:dis2020}\\
\hline
College Communities &~\cite{gong:cscw2021}\\
\hline
r/conspiracy &~\cite{samory:cscw2018,phadke:cscw2021}\\
\hline
Cryptocurrency Groups &~\cite{glenski:www2019}\\
\hline
r/dataisbeautiful &~\cite{kauer:hci2021}\\
\hline
Learning Groups &~\cite{hudgins:las2020}\\
\hline
r/lgbt &~\cite{saha:aws2019}\\
\hline
Mental Health Groups &~\cite{silveira:fgcs2021,sharma:hci2018,biester:atmis2021}\\
\hline
Misogynistic Groups &~\cite{habib:cscw2022,farrell:aws2019,farrell:aws2020}\\
\hline
North Carolina Groups &~\cite{whitfield:bcbhi2021}\\
\hline
NSFW Adult Groups &~\cite{cauteruccio:dke2022}\\
\hline
Parenting Groups &~\cite{sepahpour:www2022}\\
\hline
r/place &~\cite{israeli:www2022}\\ 
\hline
Political Groups &~\cite{massachs:aws2020,jungherr:sscr2022,chipidza:ijim2021,prakasam:isf2021}\\
\hline
Popular Groups&~\cite{wang:www2022,tuomchomtam:ida2019,thukral:asnam2020,kotenko:idaacs2021,hwang:cscw2021,park:cscw2022,zannettou:aws2020,xia:cscw2020,wood:tsc2020,urbaniak:chb2022,tsugawa:asnam2020}\\&~\cite{mall:hci2020,kumar:www2018,koncar:aws2021,kiene:cscw2019,jhaver:cscw2019,gouvea:smc2019,gadek:cwic2019,frey:cscw2022,choi:www2020,chandrasekharan:hci2018,garg:cscw2021,potts:pcc2022}\\
\hline
Post-College Groups &~\cite{saha:cscw2019}\\
\hline
Programmer Groups &~\cite{waller:www2019}\\
\hline
QAnon Groups &~\cite{engel:cscw2022}\\
\hline
r/redpill &~\cite{chandrasekharan:hci2022}\\
\hline
r/science &~\cite{williams:cscw2021,jones:hci2019}\\
\hline
r/stopsmoking &~\cite{desanto:tsc2022}\\
\hline
r/The\_Donald &~\cite{trujillo:hci2022,prakasam:isf2021,massachs:aws2020,jungherr:sscr2022,horta:cscw2021,chandrasekharan:hci2022}\\
\hline
r/Veterans &~\cite{zhou:cscw2022}\\
\hline
r/WallStreetBets &~\cite{israeli:www2022,haq:www2022}\\
\hline
Weight Loss Groups &~\cite{chancellor:hci2018,fettach:iiwbas2020}\\
\hline
r/workfromhome, r/WFH &~\cite{cho:group2022}\\
\hline
\end{tabular}
\caption{Summary of Researched \Reddit Communities}
\label{tab:redditcommunities}
\end{table*}

==> tables/redditdynamics.tex <==
\begin{table*}[!ht]
\begin{tabular}{|p{4.2cm}|p{8cm}|p{3cm}|}
\hline
\textbf{Relationship} & \textbf{Definition}  &\textbf{Related Work} \\
\hline
 Moderators and Platforms & Community bans, feature requests, and other interactions that occur between moderators and platforms &~\cite{gadek:cwic2019, juneja:group2020, matias:hci2018}\\
 \hline
 Platforms to Users & Updates, recommendations, and other interactions which platforms engage in with users &~\cite{aniche:se2018,zannettou:aws2020}\\
 \hline
 Users and Moderators & Post deletion, ban appeals, and other ways users and moderators interact&~\cite{jhaver:cscw2019, jhaver2:cscw2019, gilbert:hci2020,almerekhi:www2020, almerekhi2:www2020,horta:cscw2021,trujillo:hci2022,potts:pcc2022,juneja:group2020,seering:hci2020}\\
 \hline
 Moderator to Moderator &Direct messages, automatic mods, and other tools that facilitate interactions among moderators of a specific group&~\cite{kiene:cscw2019,dosono:hci2019,dosono:cscw2020}\\
 \hline
 User to User &Replies, direct messages, and other interactions that occur between users&~\cite{almerekhi:www2020,massachs:aws2020,jones:hci2019,hudgins:las2020,gray:dis2020,gouvea:smc2019,farrell:aws2019,farrell:aws2020,choi:www2020,williams:cscw2021,whitfield:bcbhi2021,urbaniak:chb2022,prakasam:isf2021,koncar:aws2021,chipidza:ijim2021,ng:chb2022}\\ 
 \hline
 Individual User&Posts, comments, and other interactions that a singular user engages in on a platform&~\cite{xia:cscw2020,saha:cscw2019,cho:group2022, kauer:hci2021,wood:tsc2020,waller:www2019,samory:cscw2018,saha:aws2019,hazel:sms2020,habib:cscw2022,phadke:cscw2021,mall:hci2020,kotenko:idaacs2021,engel:cscw2022,haq:www2022,gong:cscw2021,silveira:fgcs2021}\\ 
 \hline
 User and Community&The interactions that occur between a community and a member of that community&~\cite{chandrasekharan:hci2018,chancellor:hci2018,chancellor:hci2019,kotut:hci2020,fettach:iiwbas2020,zhou:cscw2022,wang:www2022,hwang:cscw2021,kauer:hci2021,cho:group2022,gauthier:hci2022,biester:atmis2021,park:cscw2022,sharma:hci2018,thukral:asnam2020,thukral:asnam2020,jungherr:sscr2022,hwang:cscw2021,decandia:aws2022,desanto:tsc2022,frey:cscw2022,garg:cscw2021}\\ 
 \hline
 Community to Community&Community migrations, cross-community harassment, and other interactions that occur between communities &~\cite{farrell:aws2019,chung:isi2019,sepahpour:www2022,mamie:aws2021,israeli:www2022,israeli:esa2022,chancellor:hci2018,gruzd:cscw2020,kumar:www2018}\\ 
 \hline
 Platform and Community&The interactions that occur between communities and platforms, such as banning entire communities&~\cite{tuomchomtam:ida2019, tsugawa:asnam2020, chandrasekharan:hci2022}\\ 
 \hline
\end{tabular}
\caption{Different Dynamics on Reddit}
\label{tab:redditdynamics}
\end{table*}
